Selective Vision-Language Subspace Projection for Few-shot CLIP

Vision-language models such as CLIP are capable of mapping the different modality data into a unified feature space, enabling zero/few-shot inference by measuring the similarity of given images and texts. However, most existing methods overlook modality gaps in CLIP's encoded features, which is shown as the text and image features lie far apart from each other, resulting in limited classification performance. To tackle this issue, we introduce a method called Selective Vision-Language Subspace Projection (SSP), which incorporates local image features and utilizes them as a bridge to enhance the alignment between image-text pairs. Specifically, our SSP framework comprises two parallel modules: a vision projector and a language projector. Both projectors utilize local image features to span the respective subspaces for image and texts, thereby projecting the image and text features into their respective subspaces to achieve alignment. Moreover, our approach entails only training-free matrix calculations and can be seamlessly integrated into advanced CLIP-based few-shot learning frameworks. Extensive experiments on 11 datasets have demonstrated SSP's superior text-image alignment capabilities, outperforming the state-of-the-art alignment methods. The code is available at https://github.com/zhuhsingyuu/SSP

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.08.  Section titles are in lowercase now.
	       Documentation updates.

Version 2.07.  Corrected typo in TELO eISSN.

Version 2.06.  Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   Changed title for TELO.

Version 2.04   Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> sections_carema-ready/deprecated.tex <==
\section{Introduction}
Vision-Language Models (VLMs) \cite{RadfordKHRGASAM21,JiaYXCPPLSLD21, LiSGJXH21} have attracted significant research interest due to their exceptional performance in various multimodal tasks \cite{ZhangGZLM0QG022, YeHRJLHYZ23, GuzhovRHD22}. Among these, CLIP (Contrastive Language-Image Pretraining) \cite{clip} stands out in classification tasks, especially in zero/few-shot scenarios. For a given test image, CLIP computes the similarity between the image feature and the text features of all class labels, in the form of \texttt{``a photo of a [class name].”}. It then assigns the class with the highest similarity as the predicted label.

\begin{figure}[t]
  \centering
    \includegraphics[width=1\linewidth]{Figs/motivation_0407.pdf}
  \caption{A illustration of modality gaps conducted on ImageNet \cite{Imagenet} with ViT-B/32. (a) Text and image features from CLIP lie in different cones. (b) Text and image features aligned by SSP almost line in the same cone. (c) Comparisons of distribution metrics for CLIP and SSP. }
  \label{fig:motivation}
\end{figure}

\begin{figure*}[!t]
  \centering
  \begin{subfigure}[b]{1\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{Figs/similarity_map_v2.pdf}
  \end{subfigure}
  \caption{Comparisons of class activations maps, where the CLIP's encoded features may concentrate on opposite or noisy regions as discussed in \cite{clipsur}, while our SSP-aligned features primarily foreground objects.}
  \label{fig:similarity_map}
\end{figure*}

Recently, prompt tuning \cite{coop, cocoop} and adapter tuning  \cite{CLIP-Adapter, tip, SuS-X} techniques have been applied in CLIP to further explore its generalization ability in few-shot tasks. These methods add learnable embeddings or adapter layers to either the visual encoder or textual encoder of CLIP. While they have improved the performance, they overlook the modality gaps existed in multi-modal models. As discussed in \cite{LFA, Gap, udandarao2022} and illustrated in Figure~\ref{fig:motivation}(a), modality gaps refer to different modality embeddings, \eg, CLIP's encoded text features (green cone) and image features (yellow cone), are located in two separated regions in a hypersphere. This phenomenon is unexpected, as paired text-image features are optimized during the pre-training stage to be closely located to each other while being separated from other paired image-text features. To further investigate these gaps, we visualize the activation maps by calculating the similarity maps between the text features and local image features (feature map) in Figure~\ref{fig:similarity_map}, the second row shows that the text features focus on the unrelated regions, not just the foreground objects. This also demonstrates the gaps between the text and image features.
In general, several reasons can cause the modality gaps, broadly categorized as follows: (1) differences in downstream dataset distribution from the training data distribution \cite{MMG}, (2) different random model initializations cause the different feature cones \cite{Gap}, (3) CLIP model does not incorporate the fine-grained relationship between text
tokens and image patches \cite{CMA-CLIP, LiuWGZFZ20}, while these works analysis the modality gaps, they do not concentrate on  CLIP's few-shot generalization capability.

Based on the observation and analysis discussed above, we propose a training-free method called \textbf{S}elective Vision-Language \textbf{S}ubspace \textbf{P}rojection (\textbf{SSP}), that leverages these local image features as a bridge to align image and text features.
Our method effectively reduces the modality gap so that the paired text-image features are no longer farther apart from each other, as shown in Figure\ref{fig:motivation}(b) ((the yellow cone and green cone are closer)).
To be specific, our SSP consists of two parallel modules, namely, a language projector and a vision projector. In the language projector module, we utilize the regions of local image features that are similar to the text feature to construct a language subspace. Subsequently, text features extracted from CLIP are aligned by projecting them onto their respective language subspaces. The vision projector module operates in a similar manner, where we use local image features to create a unified vision subspace due to the common structural and textural elements present in images, and then all image features are projected onto this vision subspace to achieve alignment. All projected features are employed to classify the test image during the inference stage.

To assess the effectiveness of our method, we take several metrics to gauge the modality gaps in CLIP and SPP. Considering both modality features have unit length and lie on a unit hypersphere, we use von Mises-Fisher (vMF) distribution \cite{banerjee2005clustering, vmf} to fit the text and image characteristics, respectively, where the parameter $\bm{\mu}$ and $\kappa$ in vMF are analogous to the mean and standard deviation of Gaussian distribution, respectively (details of vMF formalization can be found in Section Appendix).  Figure~\ref{fig:motivation}(c) summarizes the results. As expected, the text-image features aligned by SSP exhibit a higher cosine similarity, \eg, 0.7755 vs. 0.8325, as well as the smaller difference of $\kappa$, and they also obtain a closer distribution distance by comparing the KL divergence. Besides, the visualized activation maps in the last row of Figure~\ref{fig:similarity_map} show that text features processed by SSP can mainly focus on the foreground object. Overall, the above results have demonstrated the capacity of SSP to reduce gaps and improve alignment.

The main contributions of our SSP are summarized as follows:
\begin{enumerate}
\item We propose a training-free method SSP to reduce the modality gaps in CLIP's encoded features, which improves the CLIP's few-shot generalization ability.
\item We design vision and language projectors, which leverage regions of the local image features to align the image and text features via subspace projection.
\item Our SSP is flexible and can be applied to various CLIP-based methods, improving their performance across diverse benchmarks, even in state-of-the-art methods, \eg, an average accuracy improvement of 0.63\% over APE \cite{APE} in 16-shot.
\end{enumerate}

% Considering both modality features are unit length, we use von Mises-Fisher distribution \cite{banerjee2005clustering, vmf} to fit the text and image features, respectively, for gap measurements, where the parameter $\bm{\mu}$
%  is analogous to the mean of Gaussian distribution, and parameter $\kappa$  is analogous to the standard deviation of Gaussian distribution.  
 
%  Generally speaking, these modality gaps can broadly categorized into the following reasons: (1) differences in downstream dataset distribution from the training data distribution \cite{MMG}, (2) Different random model initializations cause the different cones \cite{Gap}, (3) CLIP model does not incorporate the fine-grained relationship between text
% tokens and image patches \cite{CMA-CLIP}
% As a result, in Figure~\ref{fig:similarity_map}, we visualize the activation maps by calculating the similarity maps between the text features and local image features. The second row shows that the text features focus on the unrelated regions, not just the foreground objects. These results demonstrate the existence of \textit{modality gap} in CLIP's encoded features.

% Existing zero-shot and few-shot adaption methods [x,xx,xx,x] of CLIP overlook the modality gap in v-and-t.
% The core idea of CLIP map different modality into the same space, measure the similariy to perform inference.
% modality gap is what 
% As depicted in Fig 1 left, we find that distrition gap larger, 
% consider that the image and text feauter are normalize by l2 norm,\footnote{Guassisan distribution not work,} specifically we use vMF to fit the text image ... (\mu analog to mean of gaussian, \kappa similar to std of gaussian,  details of vMF formalization can be found in Section A.) . This modality reason (1) [xx] (2) [xx](3) [xx]
% As a result, in Figure 2
% However, the CLIP model is trained on large amounts of unlabeled data obtained through web crawling ways, which often encounters mismatches in text-image pairs within this data. Additionally, directly employing a contrastive loss function to maximize the similarities of the paired text-image features and minimize the similarities of unpaired features leads to the \textit{modality gap}, as described \cite{Gap, LFA, SuS-X, udandarao2022}. Figure~\ref{fig:motivation} illustrates this phenomenon, where the top left part shows that the CLIP's encoded text and image features have unit length and lie on a unit hypersphere but in two separate regions of the shared multi-modal embedding space. However, we expect that the paired text-image features lie close together while being separated from other paired image-text features, which can make the text features to classify the test images more accurately.

% that have been discussed in the previous works \cite{LFA, Gap, udandarao2022}.
% distributional difference between encoded text features and image features, \ie, the
% either replace the handcraft prompt with learnable word embeddings or add
% Recent studies \cite{coop, tip, nips_ZhuTSZ23, aaai_ZhuNLHZ23} have further explored the generalization ability of CLIP in few-shot tasks, and adapter tuning methods \cite{CLIP-Adapter, tip, SuS-X}
% exhibit better performance compared to prompt tuning methods \cite{coop, cocoop}. Despite these advances, most existing methods have not addressed the modality gaps in CLIP's encoded text and image features. 
% As illustrated in Figure~\ref{fig:motivation}(a) and has been discussed in \cite{LFA, Gap, udandarao2022}, the text and image features are located in two completely separated regions in a hypersphere. This phenomenon differs from expectations, as the paired text-image features should be located closely together while being separated from other paired image-text features, enabling the text features to classify test images more accurately.  To further investigate these gaps, we visualize the activation maps by calculating the similarity maps between the text features and local image features in Figure~\ref{fig:similarity_map}, the second row shows that the text features focus on the unrelated regions, not just the foreground objects.
% In general, several reasons can cause the modality gaps, broadly categorized as follows: (1) differences in downstream dataset distribution from the training data distribution \cite{MMG}, (2) different random model initializations cause the different feature cones \cite{Gap}, (3) CLIP model does not incorporate the fine-grained relationship between text
% tokens and image patches \cite{CMA-CLIP, LiuWGZFZ20}, while these works do not concentrate on  CLIP's generalization capability.

 % is analogous to the mean of Gaussian distribution, and parameter $\kappa$  is analogous to the standard deviation of Gaussian distribution 

% \begin{figure}[t]
%   \centering
%   \label{fig:motivation}
%   \begin{subfigure}{0.49\linewidth}
%     \centering
%     \includegraphics[width=1\linewidth]{Figs/ViT-B32_dis_test.pdf}
%     \caption{The distributions of features extracted from CLIP.}
%     \label{fig:modality_gap}
%     \end{subfigure}
%   \begin{subfigure}{0.49\linewidth}
%     \centering
%     \includegraphics[width=1\textwidth]{Figs/ViT-B32_dis_proj_test.pdf}
%     \caption{The distributions of features projected by SSP.}
%     \label{fig:modality_gap_ssp}
%     \end{subfigure}
%    \begin{subfigure}{1\linewidth}
%     \centering
%     \includegraphics[width=1\textwidth]{Figs/motivation_hyper.pdf}
%     \caption{The text and image features lie in two separate regions without alignment by SSP.}
%     \label{fig:cone}
%    \end{subfigure}
% \captionsetup{labelformat=simple} 
%   \caption{A illustration of modality gaps in CLIP. 
%    (a) The similarity distribution of CLIP. (b) The similarity distribution of our SSP. (c) The locations of text and image features before and after alignments. 
%   }
% \end{figure}

% \begin{figure*}[!t]
%   \centering
%   \begin{subfigure}[b]{0.24\linewidth}
%     \centering
%     \includegraphics[width=0.94\linewidth]{Figs/yawl.jpg}
%     \includegraphics[width=1\linewidth]{Figs/clip_yawl.png}
%     \includegraphics[width=1\linewidth]{Figs/proj_clip_yawl.png}
%     \caption{label: ``yawl''}
%     \label{fig:RN50}
%   \end{subfigure}
%   \hfill
% \begin{subfigure}[b]{0.24\linewidth}
%     \centering
%     \includegraphics[width=0.94\linewidth]{Figs/schoolbus.jpg}
%     \includegraphics[width=1\linewidth]{Figs/schoolbus_clip.png}
%     \includegraphics[width=1\linewidth]{Figs/schoolbus_ssp.png}
%     \caption{label: ``school bus''}
%     \label{fig:RN101}
%   \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.24\linewidth}
%     \centering
%     \includegraphics[width=0.94\linewidth]{Figs/retriever.jpg}
%     \includegraphics[width=1\linewidth]{Figs/retriever_clip.png}
%     \includegraphics[width=1\linewidth]{Figs/retriever_ssp.png}
%     \caption{label: ``retriever''}
%     \label{fig:ViT-B16}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}[b]{0.24\linewidth}
%     \centering
%     \includegraphics[width=0.94\linewidth]{Figs/goose.jpg}
%     \includegraphics[width=1\linewidth]{Figs/goose_clip.png}
%     \includegraphics[width=1\linewidth]{Figs/goose_ssp.png}
%     \caption{label: ``goose''}
%     \label{fig:ViT-B32}
%   \end{subfigure}
%   \caption{Similarity maps for text feature and local image features.}
%   \label{fig:compare_fig}
% \end{figure*}

% illustrate the similarities of image-text features refined by SSP in Figure~\ref{fig:modality_gap_ssp}. We observe that the similarities of paired text-image have increased, \eg, 0.34 vs. 0.30, and similarities of unpaired text-image have decreased, \eg, 0.16 vs. 0.19. Besides, the last row of Firure\ref{fig:similarity_map} visualizes that SSP can help the text features mainly concentrating on the related object.
% Based on the above observation, our goal is to reduce the modality gap and align the paired text-image features as illustrated in Figure\ref{fig:cone}. To achieve this objective, we introduce the Selective Vision-Language Subspace Projection (SSP) method, which utilizes local image features to bridge the gap between image and text features. The SSP contains two parallel modules, the language projection, and the vision projector. The language projection module establishes a language subspace for each class by utilizing the local image features. Then, text features obtained from CLIP are aligned by projecting them onto their respective subspaces. In a similar way, the vision projector module utilizes local image features to create a shared vision subspace. All image features are then projected onto this vision subspace for alignment.

% To evaluate the effectiveness of SSP, we visualize the distribution of image-text similarities in Figure~\ref{fig:modality_gap_ssp}. We observe that the similarities of paired text-image have increased, for example, 0.34 vs. 0.30, while the similarities of unpaired text-image have decreased, for example, 0.16 vs. 0.19. Moreover, the last row of Figure\ref{fig:similarity_map} shows that SSP can help the text features to focus on the related object.



% Previous studies \cite{DenseCLIP, LoCoOp, clipsur} have demonstrated that the local image features are correlated to both vision and language.
% Consequently, to achieve this alignment, we propose \textbf{S}elective Vision-Language \textbf{S}ubspace \textbf{P}rojection (\textbf{SSP}), which leverages these local image features as a bridge to align image and text features. To be specific, our SSP consists of two parallel modules, namely, language projection and vision projector. In the language projection module, we utilize the local image features to establish a language subspace for each class. Subsequently, text features extracted from CLIP are aligned by projecting them onto their respective subspaces. The vision projector module operates in a similar manner, where we use local image features to create a shared vision subspace due to the common structural and textural elements present in images. All image features are then projected onto this vision subspace to facilitate alignment.

% Besides, the visual encoder and textual encoder of CLIP operate independently, capturing the entire image and text template, respectively, without incorporating the relationship between text tokens and image patches. These lead to the encoded text features focusing on irrelevant regions of the image, resulting in inaccurate classifications. Figure~\ref{fig:orig_act} provides an example, 
% an image belonging to the class ``\emph{yawl}'' has higher accuracy for the label ``\emph{sea}'' compared to ``\emph{yawl}'', \eg, 0.312 vs. 0.335. To illustrate this issue, we visualize the activations by measuring the similarity between the text feature and local image features, as shown in the bottom right of Figure~\ref{fig:orig_act}. We find that CLIP's text feature does not primarily focus on the object ``\emph{yawl}'' but also includes regions like ``\emph{sky}''. Conversely, our SSP method can exclusively concentrate on the ``\emph{yawl}'' object, improving classification accuracy, as depicted in Figure~\ref{fig:proj_act}.

% As illustrated in Figure~\ref{fig:compare_fig}, we obviously observe that, in the original CLIP feature space (the first row of Figure~\ref{fig:compare_fig}), the similarities of paired image-text samples only exceed slightly those of unpaired samples. While our SSP (the second row of Figure~\ref{fig:compare_fig}) effectively aligns the image-text features by reducing the similarities between unpaired image-text samples and simultaneously enhancing the similarities between paired ones, as a result, this compression of the distribution overlap leads to improved classification accuracy


